Tight Analysis of Decentralized SGD: A Markov Chain Perspective

We propose a novel analysis of the Decentralized Stochastic Gradient Descent (DSGD) algorithm with constant step size, interpreting the iterates of the algorithm as a Markov chain. We show that DSGD converges to a stationary distribution, with its bias, to first order, decomposable into two components: one due to decentralization (growing with the graph's spectral gap and clients' heterogeneity) and one due to stochasticity. Remarkably, the variance of local parameters is, at the first-order, inversely proportional to the number of clients, regardless of the network topology and even when clients' iterates are not averaged at the end. As a consequence of our analysis, we obtain non-asymptotic convergence bounds for clients' local iterates, confirming that DSGD has linear speed-up in the number of clients, and that the network topology only impacts higher-order terms.

==> sections/second-moment-bounds.tex <==
Writing the update of DGD, we have
\begin{align*}
\norm{ \globParam{t+1} - \Paramstar }^2
& =
\sum_{c=1}^\nagent 
\norm{  \locparam{c}{t+1} - \paramstar }^2
\\
& =
\sum_{c=1}^\nagent 
\bnorm{ \sum_{c'=1}^\nagent \commmat_{cc'} \Big( \locparam{c'}{t} - \paramstar - \step \ngf{c'}{ \locparam{c'}{t} } \Big) }^2
\\
& =
\sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'} 
\norm{ \locparam{c'}{t} - \paramstar - \step \ngf{c'}{ \locparam{c'}{t} }  }^2
\end{align*}
Expanding the square, we obtain
\begin{align*}
\norm{ \globParam{t+1} - \Paramstar }^2
& =
\sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'} 
\norm{ \locparam{c'}{t} - \paramstar }^2
- 2 \step
\pscal{ \ngf{c'}{ \locparam{c'}{t} }  }{ \locparam{c'}{t} - \paramstar}
+ \step^2
\norm{ \ngf{c'}{ \locparam{c'}{t} } }^2
\end{align*}
At this point, we remark that
\begin{align*}
& - 2 \step
\sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'} 
\pscal{ \ngf{c'}{ \locparam{c'}{t} }  }{ \locparam{c'}{t} - \paramstar}
\\
& \quad 
= 
- 2 \step
\sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'} 
\pscal{ \ngf{c'}{ \locparam{c'}{t} } - \ngf{c'}{ \paramstar }  }{ \locparam{c'}{t} - \paramstar}
-
2 \step
\sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'} 
\pscal{ \ngf{c'}{ \paramstar }  }{ \locparam{c'}{t} - \paramstar}
\eqsp.
\end{align*}
Therefore, we have
\begin{align*}
\norm{ \globParam{t+1} - \Paramstar }^2
& \le
\sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'} 
\Big\{ \norm{ \locparam{c'}{t} - \paramstar }^2
- 2 \step
\pscal{ \ngf{c'}{ \locparam{c'}{t} } - \ngf{c'}{\paramstar} }{ \locparam{c'}{t} - \paramstar}
+ 2 \step^2 \norm{ \ngf{c'}{ \locparam{c'}{t} } - \ngf{c'}{\paramstar} }^2 \Big\}
\\
& \qquad
+ 2 \sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'}
\Big\{  \step^2
\norm{  \ngf{c'}{\paramstar} }^2
- \step \pscal{ \ngf{c'}{ \paramstar }  }{ \locparam{c'}{t} - \paramstar}
\Big\}
\eqsp.
\end{align*}
% Which leads to the bound, using $\step \le 1/(2\lip)$,
% \begin{align*}
% \norm{ \globParam{t+1} - \Paramstar }^2
% & \le
% (1 - \step \strcvx ) \norm{ \globParam{t} - \paramstar }^2
% + 2 \sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'}
% \Big\{  \step^2
% \norm{  \ngf{c'}{\paramstar} }^2
% - \step \hetterm{c'}{t}
% \Big\}
% \eqsp.
% \end{align*}
Then we bound
\begin{align*}
2 \sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'}
\Big\{  \step^2
\norm{  \ngf{c'}{\paramstar} }^2
- \step \pscal{ \ngf{c'}{ \paramstar }  }{ \locparam{c'}{t} - \paramstar}
\Big\}
& =
2 \sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'}
\Big\{  \step^2
\norm{  \ngf{c'}{\paramstar} }^2
- \step \pscal{ \ngf{c'}{ \paramstar }  }{ \locparam{c'}{t} - \bar{\theta}_t }
\Big\}
\\
& \le
2 \sum_{c=1}^\nagent \sum_{c'=1}^\nagent \commmat_{cc'}
\Big\{  2 \step^2
\norm{  \ngf{c'}{\paramstar} }^2
+ \norm{ \locparam{c'}{t} - \bar{\theta}_t }^2
\Big\}
\eqsp.
\end{align*}
Assuming (as it should be) that $\norm{\locparam{c'}{t} - \bar{\theta}_t}^2 \le C \step^2$ for some constant $C > 0$, we obtain
\begin{align*}
\norm{ \globParam{t+1} - \Paramstar }^2
& \le
(1 - \step \strcvx) 
\norm{ \globParam{t} - \Paramstar }^2
+ 4 \step^2 \norm{ \gF{\Paramstar} }^2
+ 4 \step^2 C
\eqsp,
\end{align*}
which gives, after unrolling and taking $t$ to infinity, 
\begin{align*}
\norm{ \Paramlim - \Paramstar }^2
& \le
\frac{4 \step}{\strcvx} \Big(\norm{ \gF{\Paramstar} }^2 + C \Big)
\eqsp.
\end{align*}
